DEGREE: A Data-Efficient Generation-Based Event Extraction Model

Event extraction requires high-quality expert human annotations, which are usually expensive. Therefore, learning a data-efficient event extraction model that can be trained with only a few labeled examples has become a crucial challenge. In this paper, we focus on low-resource end-to-end event extraction and propose DEGREE, a data-efficient model that formulates event extraction as a conditional generation problem. Given a passage and a manually designed prompt, DEGREE learns to summarize the events mentioned in the passage into a natural sentence that follows a predefined pattern. The final event predictions are then extracted from the generated sentence with a deterministic algorithm. DEGREE has three advantages to learn well with less training data. First, our designed prompts provide semantic guidance for DEGREE to leverage DEGREE and thus better capture the event arguments. Moreover, DEGREE is capable of using additional weakly-supervised information, such as the description of events encoded in the prompts. Finally, DEGREE learns triggers and arguments jointly in an end-to-end manner, which encourages the model to better utilize the shared knowledge and dependencies among them. Our experimental results demonstrate the strong performance of DEGREE for low-resource event extraction.

==> 03-method_back.tex <==
\section{Data-Efficient Event Extraction}
\label{sec:method}
\begin{figure*}[t!]
    \centering
    \includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.95\textwidth]{Figures/NAACL2022_Model.pdf}
    \caption{An illustration of our method. Given an event type, we feed the model a sequence containing a passage and a set of prompts, which vary depending on the queried type.
    This figure shows the situation when the queried type is ``Contact:Attack''. 
    The model is trained to generate output texts following event-type-specific templates, which contain placeholders for filling triggers or arguments. 
    The final event predictions can made by comparing the template and the output text.}
    \label{fig:mthd_overview}
\end{figure*}

We introduce \model{}, a generation-based model for event extraction that fine-tunes BART \cite{lewis-etal-2020-bart}.\violet{here, again, I don't see any benefit of claiming `fine-tune BART'. This shouldn't be the main impression to leave to the audience about our model. I'll probably say something like `a flexible framework that formulate event extraction tasks as a natural language generation/summarization task'.}
The key idea is to design prompts to guide \model{} to generate outputs in particular formats, and the final predictions of event triggers and argument roles can be parsed from the generated outputs with a deterministic algorithm. \violet{Do we want to be more explicit to claim that our major contribution is the design of the prompts? Pros: if we explicitly claim this, we can defend this contribution by discussing the importance and the non-trivial nature of it. Cons: it may still sound trivial/simply anyway... But I feel even if we don't explicitly claim this, people will still develop that feeling.}
%Later on, the final predictions are decoded from the generated outputs.

% The key idea is to 
% generate a sentence that contains triggers and arguments from the given passage.
% The generated sentence needs to be structural so that the key information about an event (event trigger and arguments) is all retained and the final derivation of triggers and arguments from the generated sentence can be done efficiently.

As illustrated in Figure~\ref{fig:mthd_overview}, we can easily adapt to %design different prompts for 
different tasks (e.g., event detection, event argument extraction, and end-to-end EE) by altering the design of the prompts, which contain all necessary information to make predictions, such as the event type, typical event triggers, and most importantly, an \textit{event-type-specific template}.
This event-type-specific template plays a crucial role to guide the generation.
It not only provides the event structure but also defines the desired output format, which enables \model{} to capture dependencies between entities and make accurate predictions.
In the following sections, we detail our design of prompts.

% To achieve this goal, we design \textit{event-type-specific} templates to encode the unique structure of each event type.
% Given a passage and an event type, we provide the template of the queried event type to the model in order to guide \model{} to generate output in the desired format so that the final derivation can be conducted by comparing the template with the generated sentence.
% To be more specific, the input to the model is the input passage concatenated with a carefully designed \textit{prompt} with a special separator \texttt{[SEP]} in between. 
% The prompt includes elements that provide semantic information about the queried event and a predefined template for the queried event type.
% Then, the generative model is trained to output a sentence adhering to the predefined template. 
% The whole process is illustrated in Figure~\ref{fig:mthd_overview}.
\violet{This still follows the thought process of we have a pipeline ED + EAE model for EE. I think we should somehow break this by changing the writing. E.g., we can give an overview discussion saying that our goal is end-to-end EE, and it can be decomposed into the two subtasks, or not. We have design for both. But for the ease of explanation, we first introduce the two subtasks, then introduce the end-to-end design. I think this can be a major claim of our advantages -- the flexibility of the prompt design and the easiness to handle multiple subtasks in the traditional framework.}
For ease of explanation, we first introduce  \edmodel{} and \eaemodel{}, the two variants of \model{} for event detection and event argument extraction, respectively, in Section~\ref{sec:ed} and \ref{sec:eae}.
Later on, in Section~\ref{sec:e2e}, we present \model{} for end-to-end EE.

% While our focus is end-to-end event extraction, the design of our framework is general and can be applicable to subtasks of event extraction -- event trigger detection and event argument extraction by simply tweaking the prompts that are supplied to the model. 
% We use \edmodel{} and \eaemodel{} to represent the two variations. 
% For the ease of understanding, we first introduce \edmodel{} (Section~\ref{sec:ed}) and \eaemodel{} (Section~\ref{sec:eae}) and then detail our end-to-end \model{} model subsequently (Section~\ref{sec:e2e}).


\subsection{Event Detection Model}
\label{sec:ed}
Given a passage and an event type, \edmodel{} aims to exact the corresponding triggers.
The prompt of \edmodel{} contains the following:

\begin{itemize}[topsep=1pt, itemsep=-2pt, leftmargin=13pt]
    \item $\boldsymbol{\mathsf{Event\ type\ definition}}$ provides a definition for the given event type\footnote{The definition can be derived from the annotation guidelines for each dataset, e.g.\ the guideline for ACE.}. For example, \textit{``The event is related to conflict and some violent physical act.''} describes a \textit{``Conflict:Attack''} event.
    \item $\boldsymbol{\mathsf{Event\ keywords}}$ presents some words that are semantically related to the given event type. In practice, we collect three words that appear as triggers in the example sentences from the annotation guidelines. \violet{please provide examples for the Conflict:Attack event as well.}
    \item $\boldsymbol{\mathsf{ED\ template}}$ is the predefined output format for event detection tasks, which is designed as  \textit{``Event trigger is $<$Trigger$>$.''}, where \textit{``$<$Trigger$>$''} is a special token.
\end{itemize}

\noindent The goal of \edmodel{} is to generate an output text that replaces \textit{``$<$Trigger$>$''} in the \edtemp{} with the corresponding triggers.
If there are multiple possible triggers, we concatenate them with the word \textit{``and''}; if no triggers should be predicted, \edmodel{} directly copies the \edtemp{} as the output.
For example, the golden output text for \edmodel{} in Figure~\ref{fig:mthd_overview} is \textit{``Event trigger is detonated.''}, where \textit{``detonated''} is the trigger for the queried \textit{``Conflict:Attack''} type. 

\violet{Why do you have to sample? I think you should add discussion here.} When training \edmodel{}, we randomly choose $m$ event types for each example, where $m$ is a hyper-parameter.
During inference, \edmodel{} makes predictions for every event type for each example.

\subsection{Event Argument Extraction Model}
\label{sec:eae}
Given a passage and an event type as well as the corresponding trigger, \eaemodel{} identifies arguments and their roles.
The prompt of \eaemodel{} contains the following:

\begin{itemize}[topsep=1pt, itemsep=-2pt, leftmargin=13pt]
    \item $\boldsymbol{\mathsf{Event\ type\ definition}}$ is the same as the one for \edmodel{}. 
    \item $\boldsymbol{\mathsf{Query\ trigger}}$ indicates the given trigger word, as shown in Figure~\ref{fig:mthd_overview}.\violet{should probably expand the explanation rather than simply refer to the figure.}
    \item $\boldsymbol{\mathsf{EAE\ Template}}$ is an event-type-specific natural language style template. For example, in Figure~\ref{fig:mthd_overview}, the \eaetemp{} for event type \textit{``Conflict:Attack''} is \textit{``\ul{some attacker} attacked \ul{some facility, someone, or some organization} by \ul{some way} in \ul{somewhere}.''}. Each underlined part starting with \textit{``some-''} serves as a \textit{placeholder} corresponding to an argument role in an \textit{``Conflict:Attack''} event. For instance, \textit{``some way''} corresponds to the \textit{``Instrument''} role.
    Notice that every event type has it own template. 
    The full list of templates and the constructing details can be found in Appendix~\ref{sec:eaetemp_list}.
    
\end{itemize}

\noindent The objective for \eaemodel{} is to generate output texts that replace placeholders in \eaetemp{} with predicted arguments (e.g., substitute \textit{\ul{somewhere} with \textit{Gaza Strip}}).
If there are multiple arguments for the same role, they are concatenated with \textit{``and''}; if there is no predicted argument for one role, the model should copy the corresponding \textit{``some-''} in \eaetemp{}.

The \eaetemp{} plays an important role for \eaemodel{}.
First, it explicitly defines the event structure.
Second, those words starting with \textit{``some-''} provide \emph{label semantics} to help \eaemodel{} generate reasonable entities.
Finally, it controls the format of outputs.
Therefore, \eaemodel{} is able to capture dependencies between entities better and requires less training data.
Unlike previous generation-based approaches \cite{Paolini21tacl,li-etal-2020-event}, we intentionally write \eaetemp{} in natural sentence.
This makes the model easier to leverage the knowledge from pretrained decoder. In the latter section (Section~\ref{sec:ablation}), we provide experiments to demonstrate the advantage of using natural sentences.

\paragraph{Discussion} \violet{I'll probably make this more concrete by discussing our design principle for the templates (natural language, encode event structure and label semantics, you can simply refer back to the previous paragraph), and then say based on this principle, we simply came up with the current strategy without further tweak. Then you can say how long did it take for you to design the templates (instead of stating `Therefore, composing a template takes only less than 1 minute')} We want to emphasize that compared to collecting event annotations, writing templates is much easier and effortless.
As shown in Appendix~\ref{sec:eaetemp_list}, we keep the \eaetemp{} as simple and short as possible.
Therefore, composing a template takes only a few minutes.
In fact, several prior works \cite{Liu2020rceeer,Du20qa,li-etal-2020-event} also use constructed templates as weakly-supervised signals to improve models.
In Section~\ref{sec:ablation}, we will study how different templates affect the performance.


\subsection{End-to-End Event Extraction Model}\violet{if this will be our `main model', I'll spend more words on this one. Specifically, we should still have bullets for each component of this variation instead of conflating them in one paragraph.}
\label{sec:e2e}

Finally, we introduce \model~(E2E), an end-to-end event extraction model that can solve event detection and event argument extraction at the same time.
As shown in Figure~\ref{fig:mthd_overview}, the prompt of \model{} contains $\mathsf{Event\ type\ definition}$ and $\mathsf{Event\ keywords}$ as well.
In addition, we design \etoetemp{}, which is the combination of \edtemp{} and \eaetemp{}, to jointly consider triggers and arguments together.
The goal of \model{} it then to replace the placeholders in the \etoetemp{} with real triggers and arguments. 

Compared to \pipemodel{}, which combines \edmodel{} and \eaemodel{} together, \model{} is able to model the dependencies between triggers and argument. 
This is especially important when only a few training examples are available, as demonstrated in Section~\ref{sec:low_data_result}.


\subsection{Decode Predictions from Output Texts}
The process to convert output texts into final trigger and argument predictions is as follows.
We first compare the generated output with the placeholders in predefined template to determine the trigger spans and argument spans.
Next, we use directly string matching to find the offsets of the spans.
\kh{For the case that there are multiple xxx.}
